VLN-PETL: Parameter-Efficient Transfer Learning for Vision-and-Language Navigation

The performance of the Vision-and-Language Navigation~(VLN) tasks has witnessed rapid progress recently thanks to the use of large pre-trained vision-and-language models. However, full fine-tuning the pre-trained model for every downstream VLN task is becoming costly due to the considerable model size. Recent research hotspot of Parameter-Efficient Transfer Learning (PETL) shows great potential in efficiently tuning large pre-trained models for the common CV and NLP tasks, which exploits the most of the representation knowledge implied in the pre-trained model while only tunes a minimal set of parameters. However, simply utilizing existing PETL methods for the more challenging VLN tasks may bring non-trivial degeneration to the performance. Therefore, we present the first study to explore PETL methods for VLN tasks and propose a VLN-specific PETL method named VLN-PETL. Specifically, we design two PETL modules: Historical Interaction Booster (HIB) and Cross-modal Interaction Booster (CIB). Then we combine these two modules with several existing PETL methods as the integrated VLN-PETL. Extensive experimental results on four mainstream VLN tasks (R2R, REVERIE, NDH, RxR) demonstrate the effectiveness of our proposed VLN-PETL, where VLN-PETL achieves comparable or even better performance to full fine-tuning and outperforms other PETL methods with promising margins.

==> section/table_ablation.tex <==
\begin{table*}[!t]
\centering
\caption{Performance of different adaption methods on REVERIE. SPL is the main metric for its navigation task, and RGSPL is the main metric for the REVERIE task.}
\label{tab:reverie}
\vspace{-0mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c cccccc|cccccc}
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{Methods}} &Updated& \multicolumn{6}{c}{REVERIE Validation Seen} &\multicolumn{6}{c}{REVERIE Validation Unseen} &\Tstrut\\
\cline{3-20}
~&~& \multicolumn{4}{c}{Navigation}  &  \multicolumn{1}{c}{\multirow{2}{*}{RGS$\uparrow$}}&
\multicolumn{1}{c|}{\multirow{2}{*}{RGSPL$\uparrow$}} & \multicolumn{4}{c}{Navigation}  & \multicolumn{1}{c}{\multirow{2}{*}{RGS$\uparrow$}}&
\multicolumn{1}{c|}{\multirow{2}{*}{RGSPL$\uparrow$}} & \multicolumn{4}{c} \\
~&  Params(\%) &\multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{OSR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$}  & \multicolumn{1}{c}{TL} &  &  & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{OSR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} &\multicolumn{1}{c}{TL} & & & \Tstrut\\
\midrule
Fine-Tuning&100&47.15&51.37&43.97&12.92&30.71&28.63&31.70&35.79&28.44&14.79&18.18&16.24\\
\midrule
BitFit&0.80&33.52&37.81&31.84&11.45&19.96&18.93&24.65&27.46&21.34&12.36&10.85&9.43\\
Prompt Tuning&0.71&\\
LoRA&3.33&37.39&41.25&34.76&12.33&26.63&24.88&27.32&30.08&24.24&14.79&15.11&13.21\\

Adapter&3.39&\\
\midrule
VLN-PETL&3.14 \\
\bottomrule
\end{tabular}}
\vspace{-0mm}
\end{table*}
